Attention Attention Everywhere: Monocular Depth Prediction with Skip Attention

Monocular Depth Estimation (MDE) aims to predict pixel-wise depth given a single RGB image. For both, the convolutional as well as the recent attention-based models, encoder-decoder-based architectures have been found to be useful due to the simultaneous requirement of global context and pixel-level resolution. Typically, a skip connection module is used to fuse the encoder and decoder features, which comprises of feature map concatenation followed by a convolution operation. Inspired by the demonstrated benefits of attention in a multitude of computer vision problems, we propose an attention-based fusion of encoder and decoder features. We pose MDE as a pixel query refinement problem, where coarsest-level encoder features are used to initialize pixel-level queries, which are then refined to higher resolutions by the proposed Skip Attention Module (SAM). We formulate the prediction problem as ordinal regression over the bin centers that discretize the continuous depth range and introduce a Bin Center Predictor (BCP) module that predicts bins at the coarsest level using pixel queries. Apart from the benefit of image adaptive depth binning, the proposed design helps learn improved depth embedding in initial pixel queries via direct supervision from the ground truth. Extensive experiments on the two canonical datasets, NYUV2 and KITTI, show that our architecture outperforms the state-of-the-art by 5.3% and 3.9%, respectively, along with an improved generalization performance by 9.4% on the SUNRGBD dataset. Code is available at https://github.com/ashutosh1807/PixelFormer.git.

==> tables/fig-kitti.tex <==
\begin{figure*}
 \begin{center}
		\setlength\tabcolsep{2pt}
		\resizebox{0.9\textwidth}{!}{
			\renewcommand{\arraystretch}{1.1}
			\begin{tabular}{ccc}
				\includegraphics[width=0.19\linewidth]{figures/rgb1.jpg} &
				\includegraphics[width=0.19\linewidth]{figures/adabins1.png} &
				\includegraphics[width=0.19\linewidth]{figures/crf1.png} &
				\\
				\includegraphics[width=0.19\linewidth]{figures/rgb2.jpg} &
				\includegraphics[width=0.19\linewidth]{figures/adabins2.png} &
				\includegraphics[width=0.19\linewidth]{figures/crf2.png} & 
				\\
				\includegraphics[width=0.19\linewidth]{figures/rgb3.jpg} &
				\includegraphics[width=0.19\linewidth]{figures/adabins3.png} &
				\includegraphics[width=0.19\linewidth]{figures/crf3.png} &
				\\
				\includegraphics[width=0.19\linewidth]{figures/rgb_5.jpg} &
				\includegraphics[width=0.19\linewidth]{figures/adabins_5.png} &
				\includegraphics[width=0.19\linewidth]{figures/crf_5.png} &
				\\
				Input &  NeWCRFs \cite{newcrf} & Ours 
		\end{tabular}}
		\caption{Qualitative comparison of previous state-of-the-art method NeWCRFs on the outdoor dataset KITTI.}
		\vspace{-1.5em}
		\label{fig:kitti}
	\end{center}
\end{figure*}

==> tables/kittiofficial.tex <==
\begin{table*}[t]
	\centering
	\setlength{\tabcolsep}{8pt}
\begin{tabular}{lcccccccc}
\toprule
\textbf{Method}                      & \textbf{Venue}  &  \textbf{Sq Rel}$\downarrow$ & \textbf{Abs Rel}$\downarrow$ & \textbf{RMSE}$\downarrow$ & {$\log_{10}\downarrow$} & {$\delta_1\uparrow$} & {$\delta_2\uparrow$} & {$\delta_3\uparrow$}  \\                      
\midrule
Eigen \etal  \cite{eigen}           & NIPS'14              & 1.548                     & 0.203                         & 6.307                         & 0.282                                                & 0.702                        & 0.898                        & 0.967                        \\
Godard \etal \cite{Godard_2017_CVPR}            & CVPR'17              & 0.898                     & 0.114                         & 4.935                         & 0.206                                                & 0.861                        & 0.960                        & 0.976                        \\
Kuznietsov \etal \cite{Kuznietsov_2017_CVPR}        & CVPR'17              & 0.741                     & 0.113                         & 4.621                         & 0.189                                                & 0.862                        & 0.964                        & 0.986                        \\
Gan \etal \cite{gan}              & ECCV'18              & 0.666                     & 0.098                         & 3.933                         & 0.173                                                & 0.890                        & 0.984                        & 0.985                        \\
DORN \cite{dorn}                                   & CVPR'18              & 0.307                     & 0.072                         & 2.727                         & 0.120                                                & 0.932                        & 0.984                        & 0.994                        \\
Yin \etal   \cite{yinetal}           & ICCV'19              & -                         & 0.072                         & 3.258                         & 0.117                                                & 0.938                        & 0.990                        & 0.998                        \\
BTS \cite{bts}                                & Arxiv 19             & 0.245                     & 0.059                         & 2.756                         & 0.096                                                & 0.956                        & 0.993                        & 0.998                       \\
PackNet-SAN* \cite{packnetsan}                            & ICCV'21              & -                         & 0.062                         & 2.888                         & -                                                    & 0.955                        & -                            & -                            \\
TransDepth \cite{transdepth}                            & ICCV'21              & 0.252                     & 0.064                         & 2.755                         & 0.098                                                & 0.956                        & 0.994                        & 0.994                        \\
Adabins \cite{adabins}                                & CVPR'21              & 0.190                     & 0.058                         & 2.360                         & 0.088                                                & 0.964                        & 0.995                        & 0.999                        \\
DPT* \cite{dpt}                                   & ICCV'21              & -                         & 0.060                         & 2.573                         & 0.092                                                & 0.959                        & 0.995                        & 0.996                        \\
Naderi \etal \cite{naderi}            & WACV'22              &      & 0.070 & 3.223 & 0.113                        & 0.944                        & 0.991                        & \underline{0.998}                        \\
NewCRF \cite{newcrf}                                 & CVPR'22              & \underline{0.155} & \underline{0.052}     & \underline{2.129}     & \underline{0.079}                           & \underline{0.974}   & \textbf{0.997}    & 0.999    \\
\midrule
\textbf{PixelFormer (ours)} &  & \textbf{0.149}                     & \textbf{0.051}                          & \textbf{2.081}                          &  \textbf{0.077} & \textbf{0.976} & \textbf{0.997} & \textbf{0.999} \\
\bottomrule
\end{tabular}
\caption{Results on KITTI Official test set \cite{eigen}. The best results are in \textbf{bold} and second best are \underline{underlined}. ``*'' means using additional data for training. $\uparrow$ means higher the better and $\downarrow$ means lower the better. An upper bound of 80 meters on the ground truth depth map is used for evaluation.  All the numbers have been taken from the corresponding papers.  }
\label{tab:kitti}
\end{table*}

% {\bf Method} & {\bf Venue} & {\bf SILog} & {\bf sqErrorRel} & {\bf absErrorRel} & {\bf iRMSE}  \hline
% PF & & 10.36 & 1.82 \% & 8.19 \% & 10.96 & 0.1 s / 1 core & \\
% NeWCRFs \cite{newcrf} & CVPR'22 & 10.39 & 1.83 \% & 8.37 \% & 11.03 \\
% ViP-DeepLab \cite{Qiao_2021_CVPR} & CVPR'21 & 10.80 & 2.19 \% & 8.94 \% & 11.77 \\
% PWA \cite{lee} & AAAI'21 & 11.45 & 2.30 \% & 9.05 \% & 12.32 \\
% TDNet & & 11.45 & 2.17 \% & 9.20 \% & 12.02 & 0.04 s / GPU & \\
% BANet & & 11.55 & 2.31 \% & 9.34 \% & 12.17 & 0.04 s / GPU & S. Aich, J. Vianney, M. Islam, M. Kaur and B. Liu: Bidirectional Attention Network for Monocular Depth Estimation. IEEE International Conference on Robotics and Automation (ICRA) 2021.\\
% BTS & & 11.67 & 2.21 \% & 9.04 \% & 12.23 & 0.06 s / GPU & J. Lee, M. Han, D. Ko and I. Suh: From Big to Small: Multi-Scale Local Planar Guidance for Monocular Depth Estimation. 2019.\\
% DL\_61 (DORN) & & 11.77 & 2.23 \% & 8.78 \% & 12.98 & 0.5 s / GPU & H. Fu, M. Gong, C. Wang, K. Batmanghelich and D. Tao: Deep Ordinal Regression Network for Monocular Depth Estimation. IEEE Conference on Computer Vision and Pattern Recognition (CVPR) 2018.\\

==> tables/nyu_improvement.tex <==
\begin{table}
\centering
\setlength{\tabcolsep}{12pt}
\begin{tabular}{lc}
\hline
\textbf{Method} &  \textbf{\% improvement }  \\
\hline
Naderi \etal [20] & 3.9 \\
Adabins [1]  & 4.6 \\
NewCRF [34] & 7.7  \\
\hline
PixelFormer (Ours) & 5.3 \\
\hline
\end{tabular}
\caption{Improvement in performance in terms of Abs Rel against the previous SOTA for MDE on NYUV2. }
\label{tab:abl_bcp}
\vspace{-7mm}
\end{table}

                

